Introducing ROADS: A Systematic Comparison of Remote Control Interaction Concepts for Automated Vehicles at Road Works

As vehicle automation technology continues to mature, there is a necessity for robust remote monitoring and intervention features. These are essential for intervening during vehicle malfunctions, challenging road conditions, or in areas that are difficult to navigate. This evolution in the role of the human operator - from a constant driver to an intermittent teleoperator - necessitates the development of suitable interaction interfaces. While some interfaces were suggested, a comparative study is missing. We designed, implemented, and evaluated three interaction concepts (path planning, trajectory guidance, and waypoint guidance) with up to four concurrent requests of automated vehicles in a within-subjects study with N=23 participants. The results showed a clear preference for the path planning concept. It also led to the highest usability but lower satisfaction. With trajectory guidance, the fewest requests were resolved. The study's findings contribute to the ongoing development of HMIs focused on the remote assistance of automated vehicles.

==> notes.tex <==
Logging:


UserID
ScenarioID
controlMode
requestID (Nummer der Request)
elapsed Time
distanceTravelledSinceLastLog
distanceToEndOfInstructedPath (Luftlinie zum Ende des gefolgten Pfades)
lengthOfCurrentInstructedPath (Gesamtlänge noch zu folgendem gezeichneter Pfad + generierte Verbindungsstrecke Auto <-> Pfad)
lengthOfCurrentInstructedInputPath (Gesamtlänge noch zu folgendem gezeichneter Pfad)
distanceToEnd (Auto <-> Ende bis wo hin operiert werden muss)
vehiclePosition (Verlauf der unity positions vektoren -> nun auch mit offset, also vergleichbar, wenn man damit was anfangen will)
vehicleSpeed (in kmh)
constructionSiteEntered (ob erstmalig unmittelbar vor der ConstructionSite angekommen)
endReached ("Request geschafft")
closest Lane (nummer lane 0-indiziert von links bis rechts)
currentLaneDeviation (Spurabweichung zur closest Lane Mitte  auch in metern)
timeOfCollisionAvoidanceTraffic (Zeit summe wenn Verkehr in der CollisionAvoidance Range ist (egal ob hinten oder vorne, noch ob es das auto stört))
timeOfCollisionAvoidanceObstacle (wie oben für Obstacles <- Baustellenfahrzeuge, Baustellenmarker, Metallgrenzen links und rechts von Straße)
timeOfCollisionAvoidancePedestrian (wie oben für Fußgänger)
amountOfAdditionInput (Summe wie oft der Pfad erweitert wurde +1 pro Aktion)
amountOfAdditionMarkers (Summe um wie viele "Stellen" der Pfad erweitert wurde +x pro Aktion <- relevant für Anteil an Snap to Mid in Trajectory, für PathPlanning und Waypoint immer +1)
amountOfSnapToMiddleInput (+1 wenn Addition Input und mindestens einmal Snap To Mid verwendet wurde, für path planning immer 1, weil im Grunde immer Mittig)
amountOfSnapToMiddleMarkers (wie amount Of AdditionMarkers, nur dass nur hochgezählt wird wenn die "Stelle" gesnappt wurde)
amountOfReadjustmentInput (wie obiges nur statt Addition: Readjustment, heißt: anfang und ende sind in alter Trajektorie oder nah parallel dazu, Waypoint wird verschoben, PathPlanning backwards, immer +1)
timeSinceLastInput (Zeit seit letztem input)
currentlyNeglectedTime (aktuelle Zeit wie lang vehikel schon still steht (colision avoidance) oder wenn Ende vom angegebenen Pfad)
blindTimeSum (wenn vehikel nicht neglected und schon eingaben gemacht wurden -> aufsummieren Zeit wenn nicht in Main oder secondary view)
isMainRequest
isSecondaryRequest
totalRequestAmount (insgesamte Anzahl an Requests in dem Szenario, hat nicht direkt was mit dieser request instanz zu tun, aber generelle info)
sideOfConstructionSite (ob construction site links oder rechts bei der Straße




Für ein Szenario/ case jeweils::
OverviewLog:
UserID
ScenarioID
controlMode
elapsedTime
activeRequests (wie viele grade angezeigt werden)
succeededRequests (wie viele bisher geschafft sind)
mousePositionX
mousePositionY
usingMultiView (also wenn zwei Requests gleichzeitig angezeigt = true sonst = false)
usingSingleViewMain (auch nur = true wenn nur ein vehikel in der Hauptanzeige ist)
EyeGazeArea (das was du noch meintest -> was aktuell angeschaut wird: string wert aus: RequestList, MainView, SecondaryView, Instructions, None)
mouseClickLeft (summe)
mouseClickRight (summe)
pressLeftCtrl (summe)
pressShift (summe)
TimestampLog:
UserID
ScenarioID
controlMode
elapsed time
timeStampEvent (String wert aus RequestStarted, RequestFinished, RequestOpenedMain, RequestOpenedSecondary, RequestRemovedMain, RequestRemovedSecondary)
additionalInfo (eigentlich immer nur die Request Nummer des vehikels)
-> Es kommen immer Logs rein sobald eines der genannten Events auftritt. Bei den Request Opened/removed events muss man aufpassen, da jede variablen änderung geloggt wird. Demnach sind für den selben elapsedTimeTimestamp nur die Anfangs und Endzustände der jeweiligen Slots relevant.



UnitEyeLog (-> Standard Implementation) + 
 4 areas of interest definierst: links das panel mit den requests, das video mit der aktuellen Szene (ego view),  die szene top down view, und noch das Panel mit den Gründen unten
ist im OverviewLog
